Read-only Prompt Optimization for Vision-Language Few-shot Learning

In recent years, prompt tuning has proven effective in adapting pre-trained vision-language models to downstream tasks. These methods aim to adapt the pre-trained models by introducing learnable prompts while keeping pre-trained weights frozen. However, learnable prompts can affect the internal representation within the self-attention module, which may negatively impact performance variance and generalization, especially in data-deficient settings. To address these issues, we propose a novel approach, Read-only Prompt Optimization (RPO). RPO leverages masked attention to prevent the internal representation shift in the pre-trained model. Further, to facilitate the optimization of RPO, the read-only prompts are initialized based on special tokens of the pre-trained model. Our extensive experiments demonstrate that RPO outperforms CLIP and CoCoOp in base-to-new generalization and domain generalization while displaying better robustness. Also, the proposed method achieves better generalization on extremely data-deficient settings, while improving parameter efficiency and computational overhead. Code is available at https://github.com/mlvlab/RPO.

==> Section/Preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

Our approach is depicted in Figure \ref{fig:2}. We first briefly explain CLIP and CoCoOp (Conditional Context Optimization), our baseline models. Then, we present overviews of VPT (Visual Prompt Tuning), which is easily applicable to transformer based vision-language model fine-tuning.

\subsection{CLIP}

Contrastive Language Image Pre-training (CLIP) is a vision-language foundation model trained with 400M image-caption pairs. It consists of a visual encoder and a text encoder. The visual encoder takes an image as input and produces visual feature vectors, and the text encoder takes natural language text as input and outputs lingual feature vectors, which share the same latent space as visual feature vectors. 

CLIP is trained by adopting contrastive loss during the large-scale pre-training phase. Contrastive loss aims to maximize cosine similarity between matching pairs within a batch, while minimizing cosine similarity between unmatched pairs.

After pre-training, CLIP shows remarkable zero-shot classification performance on open concepts. To be specific, let $x$ and $\{t_i\}_{i=1}^{K}$ denote the image feature and the class feature extracted by CLIP. Here, $t_i$ is produced from prompts such as "A photo of a [$\mathbf{CLASS}_i$]". The prediction probability is computed as 

\begin{equation}
p(y_i|x) = \frac {\exp(sim(x, t_i)/\tau)} {\sum_{j=1}^{K} \exp(sim(x, t_j)/\tau)}
\end{equation}

where $sim(\cdot, \cdot)$ denotes cosine similarity and $\tau$ denotes the temperature parameter.\\

\subsection{Conditional Context Optimization}

Conditional Context Optimization (CoCoOp) suggests an instance of a conditional prompt tuning method which is generalizable to novel classes. 


\subsection{Visual Prompt Tuning}

Visual Prompt Tuning (VPT) is a parameter efficient fine-tuning method for Vision Transformers. It concatenates a learnable visual prompt to the input space of the Vision Transformer. The entire mechanism is formulated as,

\begin{equation} \mathbf{x^{(0)}} = [\textcolor{blue}{x^{(0)}} ; \textcolor{red}{\{p_i\}_{i=1}^{K}} ; I^{(0)}] \end{equation}

\begin{equation} \mathbf{x^{(l+1)}} = \textcolor{blue}{\mathcal{V}_{l+1}}(\mathbf{x^{(l)}}, \mathit{MASK}) \end{equation}

\begin{equation} \mathbf{x^{(L)}} = [h_0; \{z_i\}_{i=1}^{K}; I^{(L)}] \end{equation}

where $x^{(0)}$ denotes the [CLS] embedding of the pre-trained model, $P$ denotes introduced prompt embeddings and $E^{(0)} = [e_0, e_1, \ldots, e_N]$ denotes image patch embeddings. And $\mathbf{x^{(L)}}$, the final hidden representation of the [CLS] token, is used for producing classification logits. 
\\




\textbf{Our} method uses readout-only tokens to optimize the Vision-Language model. Similar to VPT, we concatenate learnable visual and text tokens to the input space of image and text encoders, and initialize them by the [CLS] token and [EOS] token respectively. We observed that by making tokens read-only and starting from a good initialization, the resulting model can effectively converge on various datasets. Masking tokens is beneficial for convergence speed and generalizability, owing to its non-disruptive behavior concerning pre-trained interactions.


==> Tables/eurosat_typo.tex <==
\begin{table}[ht]
  \centering
  \caption{EuroSAT.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CLIP    &   \textcolor{DarkGray}{56.48}   &   \textcolor{DarkGray}{64.05}   &   60.03 \\
    \midrule
    CoOp    &   \textcolor{DarkGray}{92.19}   &   \textcolor{DarkGray}{54.74}   &   68.69 \\
    CoCoOp  &   \textcolor{DarkGray}{87.49}   &   \textcolor{DarkGray}{60.04}   &   71.21 \\
    RPO     &  \textcolor{DarkGray}{88.07}   &  \textcolor{DarkGray}{68.77}   &  \textcolor{red}{\textbf{77.21}}  \\
    \bottomrule
  \end{tabular}
  \label{tab:eurosat_typo}
  \end{table}

==> Tables/supple_tab1.tex <==
\begin{table*}[t]
  % \caption{\textbf{abbab.}
  % \centering
% \setlength{\tabcolsep}{6pt}
    % abcd
  % }
\caption{\textbf{Ablation on our components in base to new generalization setting.} We evaluate base to new generalization performance by ablating read-only mask and special initialization.}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Average over 11 datasets}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{79.97} & \textcolor{DarkGray}{69.90} & 74.02 \\
    w.o init & \textcolor{DarkGray}{82.27} & \textcolor{DarkGray}{72.78} & 76.78 \\
    RPO    &   \textcolor{DarkGray}{81.13}    &   \textcolor{DarkGray}{75.00}    &   \textbf{77.78} \\
    
    \bottomrule
    \end{tabular}
    \label{tab:9.a}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{ImageNet.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{76.10} & \textcolor{DarkGray}{69.03} & 72.40 \\
    w.o init & \textcolor{DarkGray}{76.57} & \textcolor{DarkGray}{70.57} & 73.45 \\
    RPO    &   \textcolor{DarkGray}{76.60}    &   \textcolor{DarkGray}{71.57}    &   \textbf{74.00} \\
    
    \bottomrule
  \end{tabular}
  \label{tab:9.b}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Caltech101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{98.10} & \textcolor{DarkGray}{92.87} & 95.41 \\
    w.o init & \textcolor{DarkGray}{98.60} & \textcolor{DarkGray}{92.47} & 95.43 \\
    RPO    &   \textcolor{DarkGray}{97.97}    &   \textcolor{DarkGray}{94.37}    &   \textbf{96.03} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.c}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{OxfordPets.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{95.13} & \textcolor{DarkGray}{96.77} & 95.95 \\
    w.o init & \textcolor{DarkGray}{95.57} & \textcolor{DarkGray}{96.90} & \textbf{96.23} \\
    RPO    &   \textcolor{DarkGray}{94.63}    &   \textcolor{DarkGray}{97.50}    &  96.05 \\
    \bottomrule
  \end{tabular}
  \label{tab:9.d}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{StanfordCars.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{74.53} & \textcolor{DarkGray}{71.47} & 72.96 \\
    w.o init & \textcolor{DarkGray}{72.93} & \textcolor{DarkGray}{73.33} & 73.13 \\
    RPO    &   \textcolor{DarkGray}{73.87}    &   \textcolor{DarkGray}{75.53}    &   \textbf{74.69} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.e}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Flowers102.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{96.87} & \textcolor{DarkGray}{71.47} & 82.92 \\
    w.o init & \textcolor{DarkGray}{94.70} & \textcolor{DarkGray}{74.83} & 83.60 \\
    RPO    &   \textcolor{DarkGray}{94.13}    &   \textcolor{DarkGray}{76.67}    &   \textbf{84.50} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.f}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Food101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{88.97} & \textcolor{DarkGray}{88.73} & 88.85 \\
    w.o init & \textcolor{DarkGray}{90.23} & \textcolor{DarkGray}{89.87} & 90.05 \\
    RPO    &   \textcolor{DarkGray}{90.33}    &   \textcolor{DarkGray}{90.83}    &   \textbf{90.58} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.g}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{FGVCAircraft.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{35.53} & \textcolor{DarkGray}{29.90} & 32.45 \\
    w.o init & \textcolor{DarkGray}{38.37} & \textcolor{DarkGray}{31.43} & 34.55 \\
    RPO    &   \textcolor{DarkGray}{37.33}    &   \textcolor{DarkGray}{34.20}    &   \textbf{35.70} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.h}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{SUN397.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{78.96} & \textcolor{DarkGray}{76.10} & 77.50 \\
    w.o init & \textcolor{DarkGray}{80.53} & \textcolor{DarkGray}{77.60} & 79.04 \\
    RPO    &   \textcolor{DarkGray}{80.60}    &   \textcolor{DarkGray}{77.80}    &   \textbf{79.18} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.i}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{DTD.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{78.67} & \textcolor{DarkGray}{55.77} & 65.25 \\
    w.o init & \textcolor{DarkGray}{79.93} & \textcolor{DarkGray}{63.13} & \textbf{70.53} \\
    RPO    &   \textcolor{DarkGray}{76.70}    &   \textcolor{DarkGray}{62.13}    &  68.61 \\
    \bottomrule
  \end{tabular}
  \label{tab:9.j}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{EuroSAT.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{74.70} & \textcolor{DarkGray}{45.13} & 54.57 \\
    w.o init & \textcolor{DarkGray}{93.80} & \textcolor{DarkGray}{55.13} & 69.37 \\
    RPO    &   \textcolor{DarkGray}{86.63}    &   \textcolor{DarkGray}{68.97}    &   \textbf{76.79} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.k}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{UCF101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    w.o mask & \textcolor{DarkGray}{82.07} & \textcolor{DarkGray}{70.63} & 75.92 \\
    w.o init & \textcolor{DarkGray}{83.77} & \textcolor{DarkGray}{75.27} & 79.29 \\
    RPO    &   \textcolor{DarkGray}{83.67}    &   \textcolor{DarkGray}{75.43}    &   \textbf{79.34} \\
    \bottomrule
  \end{tabular}
  \label{tab:9.l}
  \end{subtable}
  \hfill
  \vspace{0.5em}
\label{tab:ablation_11}
\end{table*} 


==> Tables/supple_tab2.tex <==
\begin{table*}[h]
  % \caption{\textbf{abbab.}
  % \centering
% \setlength{\tabcolsep}{6pt}
    % abcd
  % }
\caption{\textbf{Comparison of CoCoOp, vis-RPO, text-RPO and RPO in the Base to new generalization setting.} We evaluate base to new generalization performance with unimodal RPO trained with 16-shot sampled training data.}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Average over 11 datasets}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{80.47}   &   \textcolor{DarkGray}{71.69}   &  75.83  \\
    \midrule
    text-RPO & \textcolor{DarkGray}{79.54} & \textcolor{DarkGray}{74.83} & 77.01 \\
    RPO    &   \textcolor{DarkGray}{81.13}    &   \textcolor{DarkGray}{75.00}    &   \textbf{77.78} \\
    \bottomrule
    \end{tabular}
    \label{tab:11.a}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{ImageNet.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{75.98}   &   \textcolor{DarkGray}{70.43}   &   73.10 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{76.13} & \textcolor{DarkGray}{70.70} & 73.31 \\
    RPO    &   \textcolor{DarkGray}{76.60}    &   \textcolor{DarkGray}{71.57}    &   \textbf{74.00} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.b}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Caltech101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{97.96}   &   \textcolor{DarkGray}{93.81}   &  95.84  \\
    \midrule
    text-RPO & \textcolor{DarkGray}{97.76} & \textcolor{DarkGray}{93.96} & 95.82 \\
    RPO    &   \textcolor{DarkGray}{97.97}    &   \textcolor{DarkGray}{94.37}    &  \textbf{96.03}  \\
    \bottomrule
  \end{tabular}
  \label{tab:11.c}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{OxfordPets.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{95.20}   &   \textcolor{DarkGray}{97.69}   &  \textbf{96.43} \\
    \midrule
    text-RPO & \textcolor{DarkGray}{94.56} & \textcolor{DarkGray}{97.16} & 95.84 \\
    RPO    &   \textcolor{DarkGray}{94.63}    &   \textcolor{DarkGray}{97.50}    &   96.05 \\
    \bottomrule
  \end{tabular}
  \label{tab:11.d}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{StanfordCars.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H \\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{70.49}  &   \textcolor{DarkGray}{73.59}   &   72.01 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{72.16} & \textcolor{DarkGray}{74.4} & 73.26 \\
    RPO    &   \textcolor{DarkGray}{73.87}    &   \textcolor{DarkGray}{75.53}    &  \textbf{74.69}  \\
    \bottomrule
  \end{tabular}
  \label{tab:11.e}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Flowers102.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{94.87}   &   \textcolor{DarkGray}{71.75}   &   81.71 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{91.70} & \textcolor{DarkGray}{74.90} & 82.45 \\
    RPO    &   \textcolor{DarkGray}{94.13}    &   \textcolor{DarkGray}{76.67}    &   \textbf{84.50} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.f}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{Food101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{90.70}   &   \textcolor{DarkGray}{91.29}   &   \textbf{90.99} \\
    \midrule
    text-RPO & \textcolor{DarkGray}{89.90} & \textcolor{DarkGray}{90.06} & 89.98 \\
    RPO    &   \textcolor{DarkGray}{90.33}    &   \textcolor{DarkGray}{90.83}    &   90.58
 \\
    \bottomrule
  \end{tabular}
  \label{tab:11.g}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{FGVCAircraft.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{33.41}   &   \textcolor{DarkGray}{23.71}   &   27.74 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{36.5} & \textcolor{DarkGray}{35.7} & \textbf{36.09} \\
    RPO    &   \textcolor{DarkGray}{37.33}    &   \textcolor{DarkGray}{34.20}    &  35.70  \\
    \bottomrule
  \end{tabular}
  \label{tab:11.h}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{SUN397.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{79.74}   &   \textcolor{DarkGray}{76.86}   &   78.27 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{79.56} & \textcolor{DarkGray}{77.03} & 78.27 \\
    RPO    &   \textcolor{DarkGray}{80.60}    &   \textcolor{DarkGray}{77.80}    &   \textbf{79.18} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.i}
  \end{subtable}
  \hfill
  \vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{DTD.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{77.01}   &   \textcolor{DarkGray}{56.00}   &   64.85 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{75.06} & \textcolor{DarkGray}{62.60} & 68.26 \\
    RPO    &   \textcolor{DarkGray}{76.70}    &   \textcolor{DarkGray}{62.13}    &  \textbf{68.61} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.j}
  \end{subtable}
  \hfill
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{EuroSAT.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{87.49}   &   \textcolor{DarkGray}{60.04}   &   71.21 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{79.90} & \textcolor{DarkGray}{71.60} & 75.52 \\
    RPO    &   \textcolor{DarkGray}{86.63}    &   \textcolor{DarkGray}{68.97}    &   \textbf{76.79} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.k}
  \end{subtable}
  \hfill
  %\vspace{0.5em}
  \begin{subtable}{0.3\linewidth}
  \centering
  \caption{UCF101.}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{82.33}   &   \textcolor{DarkGray}{73.45}   &   77.64 \\
    \midrule
    text-RPO & \textcolor{DarkGray}{81.70} & \textcolor{DarkGray}{75.1} & 78.26 \\
    RPO    &   \textcolor{DarkGray}{83.67}    &   \textcolor{DarkGray}{75.43}    &   \textbf{79.34} \\
    \bottomrule
  \end{tabular}
  \label{tab:11.l}
  \end{subtable}
  \hfill
  \vspace{0.5em}
\label{tab:uni_rpo_11}
\end{table*} 


==> Tables/supple_tab3.tex <==
\begin{table*}[t]
    \centering
    \caption{\textbf{Evaluation of robustness and base to new generalizability.} We trained RPO and CoCoOp on 16-shot learning setting with 10 random seeds. mean denotes harmonic mean averaged over 10 random seeds and std denotes standard deviation of the 10 harmonic means.}
    \begin{tabular}{l@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc@{\hspace{\tabcolsep}}cc}
        \toprule
        & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{FGVCAircraft}& \multicolumn{2}{c}{DTD} & \multicolumn{2}{c}{StanfordCars} & \multicolumn{2}{c}{UCF101} & \multicolumn{2}{c}{Flowers102}   \\
          \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-7}\cmidrule(r){8-9}\cmidrule(r){10-11}\cmidrule(r){12-13}\cmidrule(r){14-15} 
          &{CoCoOp} & {RPO} & {CoCoOP} & {RPO} & {CoCoOp} & {RPO} & {CoCoOp} & {RPO}& {CoCoOp} & {RPO}& {CoCoOp} & {RPO}\\
          \cmidrule(r){1-15}
        mean  & 73.65 & \textbf{74.38}  & 28.88 & \textbf{36.09} & 62.74 & \textbf{68.43} & 72.14 & \textbf{74.18} & 77.53& \textbf{79.75} & 81.42 & \textbf{84.23}\\
        std & 13.64 & \textbf{3.48} & 10.52 & \textbf{0.58} & 2.87 & \textbf{1.05} & 0.60 & \textbf{0.32} & 1.02 & \textbf{0.52} & 0.95 & \textbf{0.51}  \\
    \bottomrule
  \end{tabular}
  \label{tab:variance_analysis}
\end{table*}

==> Tables/table10.tex <==
\begin{table}[ht]
    \centering
    \caption{\textbf{Analysis of the computational efficiency of RPO compared to CoCoOp.}}
    \begin{subtable}{1.0\linewidth}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & \ $\#$ params & Complexity  & MAC \\
    \midrule
    CoCoOp  &   $35,360$   &  $O(CN_t^2 + N_v^2)$   & \\
    \textbf{RPO}   &   $30,720$    &  $O(N_v^2)$   & \\
    \bottomrule
    \end{tabular}
  \end{subtable}
  \label{tab:10}
\end{table}

==> Tables/table5.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Analysis of the computational efficiency of RPO compared to CoCoOp and CoOp.} RPO is much lighter than CoCoOp from the standpoint of the number of parameters and inference speed, meanwhile resolving the generalization problem of CoOp.}
    \begin{subtable}{1.0\linewidth}
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & \ $\#$ params & Complexity & H.M(\%) \\
    \midrule
    CoOp  &  $2,048$   &  $O(CN_t^2 + BN_v^2)$  & 71.66\\
    CoCoOp  &   $35,360$   &  $O(BCN_t^2 + BN_v^2)$  & 75.83\\
    \textbf{RPO}   &   $30,720$    &  $O(CN_t^2 + BN_v^2)$  & \textbf{77.77}\\
    \bottomrule
    \end{tabular}
  \end{subtable}
  \label{tab:5}
\end{table}

==> Tables/table7.tex <==
\begin{table}[hbt!]
    \centering
    \caption{\textbf{Comparison between RPO with original attention mask and variant attention mask} We achieve better generalizability by applying variant attention mask within the framework of RPO.}
    %We observed that without attention mask and prompt initialization, %performance largely varies depending on random seed, especially on %small scale datasets. i.e. EuroSAT, Describable Textures Dataset. We %represent this phenomenon by evaluate models on small datasets on %various seeds.

    \begin{subtable}{0.9\linewidth}
  \begin{tabular}{c|c|c|c}
    \toprule
    Method &Base & Novel & H\\
    %\cmidrule(r){2-2}
    %& Init  Mask & & &\\
    \midrule
    CoCoOp &  80.92   & 71.82  &  75.67  \\
            RPO (original) &     82.06    &   73.44   &   77.07 \\
            RPO (variant) &     \textbf{82.35}    &   \textbf{74.06}   &   \textbf{77.65}\\
    \bottomrule
    \end{tabular}
  \end{subtable}
  \label{tab:7}
\end{table}



==> Tables/table8.tex <==
\begin{table}[h]
  % \caption{\textbf{abbab.}
  % \centering
% \setlength{\tabcolsep}{6pt}
    % abcd
  % }
\caption{\textbf{Results on intra-task generalization and ablation averaged over 11 datasets.} }
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    Methods & Base & Novel & H\\
    \midrule
    CoCoOp  &   \textcolor{DarkGray}{80.47}   &   \textcolor{DarkGray}{71.69}   &   75.83 \\
    RPO w.o mask & \textcolor{DarkGray}{79.97} & \textcolor{DarkGray}{69.90} & 74.02 \\
    RPO w.o init & \textbf{\textcolor{DarkGray}{82.27}} & \textcolor{DarkGray}{72.78} & 76.78 \\
    uni-RPO & \textcolor{DarkGray}{80.23} & \textcolor{DarkGray}{74.98} & 77.38 \\
    RPO    &   \textcolor{DarkGray}{81.13}    &   \textbf{\textcolor{DarkGray}{75.01}}    &   \textbf{77.77} \\
    
    \bottomrule
    \end{tabular}
\label{tab:1}
\end{table} 

